CONFINE: Preserving Data Secrecy in Decentralized Process Mining

In the contemporary business landscape, collaboration across multiple organizations offers a multitude of opportunities, including reduced operational costs, enhanced performance, and accelerated technological advancement. The application of process mining techniques in an inter-organizational setting, exploiting the recorded process event data, enables the coordination of joint effort and allows for a deeper understanding of the business. Nevertheless, considerable concerns pertaining to data confidentiality emerge, as organizations frequently demonstrate a reluctance to expose sensitive data demanded for process mining, due to concerns related to privacy and security risks. The presence of conflicting interests among the parties involved can impede the practice of open data sharing. To address these challenges, we propose our approach and toolset named CONFINE, which we developed with the intent of enabling process mining on process event data from multiple providers while preserving the confidentiality and integrity of the original records. To ensure that the presented interaction protocol steps are secure and that the processed information is hidden from both involved and external actors, our approach is based on a decentralized architecture and consists of trusted applications running in Trusted Execution Environments (TEE). In this demo paper, we provide an overview of the core components and functionalities as well as the specific details of its application.

==> content/addon/pkgloading.tex <==
% For language-specific hyphenations etc.
\usepackage[english]{babel}
% For subfigures
\usepackage{subcaption}
\usepackage{xcolor}
% For nice links
\usepackage{url}
% For playing with colors in tabular environments
\usepackage{colortbl}
% For math symbols, such as \nexists
\usepackage{amssymb}
% For more math symbols, such as \mapsfrom
\usepackage{stmaryrd}
% For advanced graphics
% For equations, arrays of equations, defining operator names, etc.
\usepackage{amsmath}
% For cursive math
\usepackage{mathrsfs}
% For math symbols, such as \nexists
\usepackage{amssymb}
%% For math environments, such as "definition"
\usepackage{amsthm}
\theoremstyle{definition}
\newdefinition{definition}{Definition}[section]
\newtheorem{theorem}{Theorem}[section]
\newtheorem{assumption}{Postulate}[section]
\newtheorem{proposition}{Proposition}[section]
% For enumerating the line numbers
\usepackage[left]{lineno}
% For diagonally-split fractions (\sfrac)
\usepackage{xfrac}
% For nice (diagonal) fractions
\usepackage{nicefrac}
% For side notes, missing figures and inline to-do's
\usepackage[textsize=scriptsize,backgroundcolor=yellow!40]{todonotes}
% Resize the width of todo-notes on the margins
%\setlength{\marginparwidth}{1.25cm}
% For specifying kewords and acronyms
\usepackage[nonumberlist,acronym,sanitize=none]{glossaries}
\glsdisablehyper
% For commenting out some parts of the text
\usepackage{comment}
% For hyperlinks
\usepackage[pdftex, colorlinks=true, hyperfootnotes=true, hyperindex=true,
            plainpages=false, pagebackref=false, pdfpagelabels=true, pdfstartview=FitH,
            linkcolor=blue, citecolor=blue, urlcolor=blue,
            bookmarks, bookmarksopen, bookmarksdepth=3]{hyperref}
% For smart references
\usepackage[capitalise,nameinlink]{cleveref}
% To have "Figure 3(a)" in place of "Figure 3a" and  "Table 3(a)" in place of "Table 3a"
\captionsetup[subfigure]{subrefformat=simple,labelformat=simple}
    \renewcommand\thesubfigure{(\alph{subfigure})}
\captionsetup[subtable]{subrefformat=simple,labelformat=simple}
    \renewcommand\thesubtable{(\alph{subtable})}
\crefname{algocf}{Alg.}{Algs.}
\Crefname{algocf}{Algorithm}{Algorithms}
\crefname{definition}{Def.}{Defs.}
\Crefname{definition}{Definition}{Definitions}
\crefname{assumption}{Post.}{Posts.}
\Crefname{assumption}{Postulate}{Postulates}
\crefname{aAlgocflLine}{line}{lines}
\Crefname{algocfline}{Line}{Lines}
\crefname{section}{Sect.}{Sects.} % Era un poco prolisso
\crefname{Section}{Section}{Sections} % Era un poco prolisso
% TikZ/Pgf advanced graphics
\usepackage{tkz-base}
\usetikzlibrary{decorations.pathmorphing,trees,snakes,arrows,shapes,automata,petri}
% To use inline and other fancy list-like environments (e.g., inparaenum)
\usepackage{paralist}
% To divide a text line into multiple columns
\usepackage{multicol}
% To create good-looking book-style tables
\usepackage{booktabs}
% To play around with list environments
\usepackage{enumitem}
% To create multirow cells in tables
\usepackage{multirow}
% To create rotated cells in tables
\usepackage{rotating}
% To create enumerated lists, whose numbering is reversed
\usepackage{etaremune}
%% To make algorithmic nice-looking pseudocode
\usepackage[ruled,linesnumbered,algo2e]{algorithm2e}
\SetCommentSty{textrm} % Avoid that comments are written in teletype text: it consumes loads of space!
\SetArgSty{textrm} % Avoid that arguments are in italic. It barely ever serves the purpose!
\SetFuncArgSty{textrm} % Avoid that fuction arguments are in italic. It barely ever serves the purpose!
\renewcommand{\SetProgSty}[1]{\renewcommand{\ProgSty}[1]{\textnormal{\csname#1\endcsname{##1}}\unskip}}% https://tex.stackexchange.com/questions/701459/how-to-set-the-kwprog-arg-font-style-with-something-like-setprogsty-in-algori
\SetProgSty{textrm} % Avoid that program arguments are in italic. It barely ever serves the purpose!
%% For creating side-notes
\usepackage{marginnote}
% For superimposing symbols over one another within math env.
\usepackage{mathtools}
% For strange math symbols like \Dashv
\usepackage{mathabx}
% For adjusting the size of tables to the text width, if necessary: \begin{adjustbox}{max width=\textwidth}
\usepackage{adjustbox}
% For LaTeX if/then statements
\usepackage{ifthen}
% For strike-through cancellations
\usepackage[normalem]{ulem}
%% The lineno packages adds line numbers. Start line numbering with
%% \begin{linenumbers}, end it with \end{linenumbers}. Or switch it on
%% for the whole article with \linenumbers.
\usepackage{lineno}
% For highlighted text
\usepackage{soul}
% To put table environments and co. side by side
\usepackage{floatrow}
\floatsetup[table]{style=plaintop}
\usepackage{listings}
\begin{comment}
	contenuto...
\lstset{ %
%	backgroundcolor=\color{white},   % choose the background color; you must add \usepackage{color} or \usepackage{xcolor}; should come as last argument
	basicstyle=\tiny\ttfamily,       % the size of the fonts that are used for the code
	breakatwhitespace=true,          % sets if automatic breaks should only happen at whitespace
	breaklines=true,                 % sets automatic line breaking
	captionpos=b,                    % sets the caption-position to bottom
	commentstyle=\color{gray},       % comment style
%	escapeinside={\%*}{*)},          % if you want to add LaTeX within your code
	extendedchars=true,              % lets you use non-ASCII characters; for 8-bits encodings only, does not work with UTF-8
	frame=single,	                 % adds a frame around the code
	keepspaces=true,                 % keeps spaces in text, useful for keeping indentation of code (possibly needs columns=flexible)
%	keywordstyle=\color{blue},       % keyword style
%	language=SQL,                    % the language of the code
%	deletekeywords={Time},      % if you want to delete keywords from the given language
%	morekeywords={*,...},            % if you want to add more keywords to the set
	numbers=left,                    % where to put the line-numbers; possible values are (none, left, right)
	numbersep=5pt,                   % how far the line-numbers are from the code
	numberstyle=\tiny\color{gray}, % the style that is used for the line-numbers
%	rulecolor=\color{black},         % if not set, the frame-color may be changed on line-breaks within not-black text (e.g. comments (green here))
	showspaces=false,                % show spaces everywhere adding particular underscores; it overrides 'showstringspaces'
	showstringspaces=false,          % underline spaces within strings only
	showtabs=false,                  % show tabs within strings adding particular underscores
	stepnumber=1,                    % the step between two line-numbers. If it's 1, each line will be numbered
%	stringstyle=\color{mymauve},     % string literal style
	tabsize=2,	                   % sets default tabsize to 2 spaces
%	title=\lstname                   % show the filename of files included with \lstinputlisting; also try caption instead of title
	morecomment=[l]\%
}
\end{comment}

\lstset{
	backgroundcolor=\color{scriptcolor},
	extendedchars=true,
	basicstyle=\fontsize{8pt}{8pt}\selectfont\ttfamily,
	showstringspaces=false,
	showspaces=false,
%	linewidth=19em,
	numbers=left,
	numberstyle=\footnotesize,
	numbersep=5pt,
	tabsize=2,
	breaklines=true,
	showtabs=false,
	captionpos=b,
	%belowskip=-0.2em,
	lineskip = 0.1em
}
\crefname{lstlisting}{Listing}{Listings}
% To add dummy text
\usepackage{lipsum}
% To have newlines in cells, with commands such as \makecell or \thead
\usepackage{makecell}
% For diagonal lines in tables
\usepackage{diagbox}
% For a decent formatting of numbers (and a wonderful system for numeric columns in tables, ``S'')
\usepackage[scientific-notation=false,group-separator={,}]{siunitx}
% To enable text protrusion
\usepackage{microtype}
% For footnote-references: \footref
\usepackage{footmisc}
% For side figures
\usepackage{wrapfig}
%
%\usepackage{xcolor}

\usepackage[ddmmyyyy]{datetime}
\usepackage{scrextend}
\usepackage{textcase}
\usepackage{setspace}

==> content/addon/squeeze.tex <==
%% Saving trees -- put this in the preamble
\usepackage{newtxtext}
%% Do not let the Times package affect the monospaced font (Courier is utterly ugly)
\renewcommand{\ttdefault}{cmtt}
%% Shrinking white space here and there…
\usepackage[subtle]{savetrees}
%\addtolength{\topmargin}{-1\baselineskip} % Careful!
%\addtolength{\textheight}{2\baselineskip} % Careful!
%% save space around floats (tables, algo's, fig's):
\setlength{\textfloatsep}{15pt}% Reduce \textfloatsep
%% save more space by suppressing vertical space between paragraphs
%\parskip1pt

==> content/addon/utils.tex <==
% Additional macros for algorithm2e
% Requires:
%   \usepackage[...]{algorithm2e}
\SetKw{Trigger}{trigger}
\SetKw{Yield}{yield}
\SetKw{Return}{return}
\SetKwProg{UponEv}{upon event}{ do}{}
\SetKwProg{Upon}{upon}{ do}{}
\SetKwInput{Implements}{Implements}
\SetKwInput{Uses}{Uses}
\SetKwProg{Fn}{Function}{ is}{}
\def\self {\ensuremath{\textrm{self}}}
\newcommand{\Mesg}[1]{\ensuremath{\textrm{\textsc{#1}}}}
\newcommand{\SuchThat}[1]{~\textrm{\textbf{such that}}~{#1}}
\newcommand{\To}[1]{~\textrm{\textbf{to}}~{#1}}
\newcommand{\Call}[1]{\texttt{#1}}

% Creates a smart reference to an algorithm pseudocode block (1st parameter, OPTIONAL, in square brackets) and line (2nd parameter)
% Requires:
%  \usepackage[capitalise,nameinlink]{cleveref}
%  \crefname{algocf}{Alg.}{Algs.}
%  \Crefname{algocf}{Algorithm}{Algorithms}
%  \usepackage{xparse}
\DeclareDocumentCommand{\crefalgln}{ o m }{%
	\IfNoValueF{#1}{\cref{#1}, }% if the first optional parameter is passed, print the reference to the algorithm
	{\hyperref[#2]{ln.~\ref{#2}}}% Print the line number with reference
}%
% Usage examples:
%   \crefalgln[alg:lprv]{alg:lprv:CasesRefReq} → Alg. 2, Line 1
%   \crefalgln{alg:lprv:CasesRefReq} → Line 1

% Def-eq
%\newcommand*{\defeq}{\ensuremath{\;\stackrel{\text{def}}{=}\;}}

==> content/motivating.tex <==
\def\Talice{\Activ{PH, COPA, OD, \color{pharmacolor}DOR, PDL, SD, \color{black}RD, AD, TP, \color{specializedcliniccolor}PAFH, PIA, PT, VRT, TPB, \color{black}RPB, DPH, PCD, DP}}
\def\Tbob{\Activ{PH, COPA, OD, \color{pharmacolor}DOR, PDL, SD, \color{black}RD, AD, PRTA, PCD, DPH, DP}}
\def\TaliceUncolored{\Activ{PH, COPA, OD, DOR, PDL, SD, RD, AD, TP, PAFH, PIA, PT, VRT, TPB, RPB, DPH, PCD, DP}}
\def\TbobUncolored{\Activ{PH, COPA, OD, DOR, PDL, SD, RD, AD, PRTA, PCD, DPH, DP}}
\begin{figure}[t]
\centering

%\includegraphics[width=0.9\linewidth]{content/figures/healthcarescenario.pdf}
\includegraphics[width=\linewidth]{content/figures/bpmnHealthcare2.pdf}
\caption{A BPMN collaboration diagram of a simplified healthcare scenario}
\label{fig:BPMN_Healthcare}
\end{figure}
\begin{table}[t]%\hskip-2.5cm
  \caption{Events from cases 312 (Alice) and 711 (Bob) recorded by the \Actor{Hospital}, the \Actor{Specialized clinic}, and the \Actor{Pharmaceutical company}}
 \centering
    \begin{minipage}[c]{0.55\linewidth}
    %\subfloat{% Subtable 1
       \resizebox{0.99\textwidth}{!}{% <------ Don't forget this %
        \begin{tabular}{ll|l|l|l|l|l|l|}
        
        & \multicolumn{7}{c}{\large{\textbf{Hospital}}\vspace{0.2em}}                                               \\ \cline{2-4}\cline{6-8}
        \multicolumn{1}{c|}{} & {Case} & {Timestamp} & Activity &  & {Case} & {Timestamp} & Activity \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_1$} & {312}         & {2022-07-14T10:36}           & PH    & $\Evt_{11}$ & {312}         & {2022-07-15T22:06}           & TP     \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_2$} & {312}         & {2022-07-14T16:36}           & COPA  & $\Evt_{12}$ &  {711}         & {2022-07-16T00:55}           & PRTA          \\ \cline{2-4} \cline{6-8} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_3$} & {711}         & {2022-07-14T17:21}           & PH    & $\Evt_{13}$ &  {711}         & {2022-07-16T01:55}           & PCD            \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_4$} & {312}         & {2022-07-14T17:36}           & OD    & $\Evt_{14}$ &  {711}         & {2022-07-16T02:55}           & DPH           \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_5$} & {711}         & {2022-07-14T23:21}           & COPA  & $\Evt_{15}$ &  {711}         & {2022-07-16T04:55}           & DP          \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_6$} & {711}         & {2022-07-15T00:21}           & OD    & $\Evt_{16}$ &   {312}         & {2022-07-16T07:06}           & RPB        \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_7$} & {711}         & {2022-07-15T18:55}           & RD    & $\Evt_{17}$ &   {312}         & {2022-07-16T09:06}           & DPH          \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_8$} & {312}         & {2022-07-15T19:06}           & RD    & $\Evt_{18}$ &   {312}         & {2022-07-16T10:06}           & PCD         \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_9$} & {711}         & {2022-07-15T20:55}           & AD    & $\Evt_{19}$ &   {312}        & {2022-07-16T11:06}           & DP            \\ \cline{2-4} \cline{6-8}
        \multicolumn{1}{c|}{$\Evt_{10}$} & {312} & {2022-07-15T21:06}           & AD \\ \cline{2-4}
        \end{tabular}%
        \label{tab:partitions}
        }% resizebox
    %}% subfloat
    \end{minipage}%
    \hspace{0.004\textwidth}%
    \begin{minipage}[c]{0.33\linewidth}
    %\subfloat[Specialised Clinic]{\label{tab:testResults:decentralized}% Subtable 2
    %\subfloat{% Subtable 2
        \resizebox{\textwidth}{!}{% <------ Don't forget this %
            \raisebox{2\baselineskip}{%
                \begin{tabular}{ll!{\color{pharmacolor}\vline}l!{\color{pharmacolor}\vline}l!{\color{pharmacolor}\vline}}\arrayrulecolor{pharmacolor}
                & \multicolumn{3}{c}{\large{\textbf{Pharmaceutical company}}\vspace{0.2em}}                                               \\ \cline{2-4}
                \multicolumn{1}{c|}{}&{HospitalCaseID} & {Timestamp} & Activity \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{20}$} &312          & {2022-07-15T09:06}           & DOR \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{21}$} &711         & {2022-07-15T09:30}           & DOR \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{22}$} &312         & {2022-07-15T11:06}           & PDL \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{23}$} &711         & {2022-07-15T11:30}           & PDL \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{24}$} &312         & {2022-07-15T13:06}           & SD  \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{25}$} &711          & {2022-07-15T13:30}           & SD  \\ \cline{2-4}
                \end{tabular}%
            }% raisebox
        }% resize box
     %\end{minipage}%<
        %\hspace{0.005\textwidth}
        \\[0.3em]
     %\begin{minipage}[t]{0.49\linewidth}
        \resizebox{\textwidth}{!}{% <------ Don't forget this %
            \raisebox{2.5\baselineskip}{%
                \begin{tabular}{ll!{\color{specializedcliniccolor}\vline}l!{\color{specializedcliniccolor}\vline}l!{\color{specializedcliniccolor}\vline}}\arrayrulecolor{specializedcliniccolor}
        
                & \multicolumn{3}{c}{\large{\textbf{Specialized clinic}}\vspace{0.2em}}                                               \\\cline{2-4}
                \multicolumn{1}{c|}{} & {TreatmentID}  & {Timestamp} & Activity \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{26}$}&312         & {2022-07-16T00:06}           & PAFH        \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{27}$}&312          & {2022-07-16T01:06}           & PIA         \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{28}$}&312          & {2022-07-16T03:06}           &  PT         \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{29}$}&312          & {2022-07-16T04:06}           & VRT         \\ \cline{2-4}
                \multicolumn{1}{c|}{$\Evt_{30}$}&312          & {2022-07-16T05:06}           & TPB         \\ \cline{2-4}
                \end{tabular}%
            }% raisebox
        }% resizebox
    \end{minipage}
    \\[0.3em]
    \begin{minipage}[t]{\linewidth}
            \resizebox{\textwidth}{!}{%
                \begin{tabular}{p{18cm}}
                $T_{312}=${\textlangle}  \Talice \,{\textrangle}\\[0.5\baselineskip]
                $T_{711}=${\textlangle}  \Tbob \,{\textrangle}\\
                \end{tabular}%
                     \label{tab:trace}
            }% resizebox
\end{minipage}
    \end{table}


\section{Motivating Scenario}
\label{sec:scenario}

For our motivating scenario, we focus on a simplified hospitalization process for the treatment of rare diseases.
The process model is depicted as a BPMN diagram in \cref{fig:BPMN_Healthcare} and involves the cooperation of three parties: a \Actor{Hospital}, a \Actor{Pharmaceutical company}, and a \Actor{Specialized clinic}.
For the sake of simplicity, we describe the process through two cases, recorded by the information systems as in \cref{tab:partitions}. 
Each patient in the hospital is associated with an id which would be the identifier of the case in the hospital log.

\begin{comment}
    

%Alice's journey %(\textbf{case 312})
begins when she enters the hospital for the preliminary examinations (patient hospitalized, \Activ{PH}). The \Actor{Hospital} then places an order for the drugs (\Activ{OD}) to the \Actor{Pharmaceutical company} for  treating Alice's specific condition. Afterwards, the \Actor{Pharmaceutical company} acknowledges that the drugs order is received (\Activ{DOR}), proceeds to produce the drugs in the laboratory (\Activ{PDL}), and ships the drugs (\Activ{SD}) back to the \Actor{Hospital}. Upon receiving the medications, the \Actor{Hospital} administers the drug (\Activ{AD}), and conducts an assessment to determine if Alice can be treated internally. If specialized care is required, the \Actor{Hospital} transfers the patient (\Activ{TP}) to the \Actor{Specialized clinic}. When the patient arrives from the hospital (\Activ{PAFH}), the \Actor{Specialized clinic} performs in-depth analyses (\Activ{PIA}) and proceeds with the treatment (\Activ{PT}). Once the \Actor{Specialized clinic} had completed the evaluations and verified the response to the treatment (\Activ{VRT}), it transfers the patient back (\Activ{TPB}). The \Actor{Hospital} receives the patient back \Activ(RPB) and prepares the clinical documentation (\Activ{PCD}). If Alice has successfully recovered, the \Actor{Hospital} declares the patient as healed (\Activ{DPH}). When Alice's treatment is complete, the \Actor{Hospital} discharges the patient (\Activ{DP}). 
%
Bob %(\textbf{case 711}) 
enters the \Actor{Hospital} a few hours later than Alice. His hospitalization process is similar to Alice's. However, he does not need specialized care, and his case is only treated by the \Actor{Hospital}. Therefore, the \Actor{Hospital} performs the response to treatment analyses (\Activ{PRTA}) instead of transferring him to the \Actor{Specialized clinic}. 
\end{comment}


Both the National Institute of Statistics of the country in which the three organizations reside and the University that hosts the hospital wish to uncover information on this inter-organizational process for reporting and auditing purposes~\citep{Jans.Hosseinpour/IJAIS2019:ActiveLearningProcessMiningForAuditing} via process analytics. The involved organizations share the urge for such an analysis and wish to be able to repeat the mining task also in-house. 
The \Actor{Hospital}, the \Actor{Specialized clinic}, and the \Actor{Pharmaceutical company} have a partial view of the overall unfolding of the inter-organizational process as they record the events stemming from the parts of their pertinence. %They record the events, e.g., of Alice and Bob's hospitalizations on traces 312 and 711 % of their event logs respectively, 
%alongside traces associated with other patients. 

{In \cref{tab:partitions}, we show Alice and Bob's cases (identified by the \textbf{312} and \textbf{711} codes respectively) recorded by the  by the \Actor{Hospital} (i.e., $T^H_{312}$ and $T^H_{711}$), the \Actor{Specialized clinic} (i.e., $T^S_{312}$ and $T^S_{711}$), and the \Actor{Pharmaceutical company} (i.e., $T^C_{312}$ and $T^C_{711}$). The \Actor{Hospital} stores the identifier of these cases in the \textit{case} id attribute of its event log. Differently, the \Actor{Specialized clinic} and the \Actor{Pharmaceutical company} employees a different case denomination and stores the cross-organizational identifiers in other attributes (\textit{`TreatmentID}' and \textit{`HospitalCaseID}' respectively).}  %The identification number is assigned to patients by the \Actor{Hospital}. 
% In order to gain valuable insights concerning the whole hospitalization process, the \Activ{Hospital} retrieves event logs from the \Actor{Specialized clinic} and the \Actor{Pharmaceutical company}. These include $T_{S312}$, $T_{C312}$, $T_{S711}$, $T_{C711}$. The \Activ{Hospital} combines its traces with those sharing the same id from the \Actor{Specialized clinic} and the \Actor{Pharmaceutical company}. The results of this procedure are chronologically sorted traces that encompass the events of the three organizations. Therefore, the \Actor{Hospital} combines $T_{H312}, T_{C312}, T_{S312}$ and $T_{H711}, T_{C711}, T_{S711}$ generating 
 The partial traces of the three organizations are projections of the two combined ones for the whole inter-organizational process: $T_{312}=$\textlangle{}{\TaliceUncolored}\textrangle{} and $T_{711}=$\textlangle{}{\TbobUncolored}\textrangle{}. %Merged traces are used by the \Actor{Hospital} as input of the HeuristicsMiner~\citep{heuristicsminer} algorithm that outputs the business model of the whole process. Finally, the \Actor{Hospital} employs the outputs of the algorithm to uncover hidden process insights, revealing patterns, deviations, and opportunities for optimization within the hospitalization routine. 
Results stemming from the analysis of the local cases would not provide a full picture. Data should be merged. However, to preserve the privacy of the people involved and safeguard the confidentiality of the information, the involved parties \textit{cannot give open access to their traces to other organizations}. The diverging interests (being able to conduct process mining on data from multiple sources without giving away the local event logs in-clear) motivate our research. In the following, we describe the design of our solution. 


==> content/related.tex <==
\label{sec:related}
\section{Related Work}

==> content/tables/coefficentsTestTable.tex <==
\begin{subfigure}{0.49\textwidth}
\label{tab:metrics}
  \centering
   \subfloat[Scalability metrics]{%
   \resizebox{0.94\textwidth}{!}{%
    \begin{tabular}{l c c c c}
       \toprule
         & \textbf{Linear Corr}.  & \textbf{Linear Slope}  & \textbf{R$^2$} & \textbf{Speedup}\\
         \midrule
         \multicolumn{5}{c}{\textbf{Number of cases test}} \\
         \midrule
         Seg. size 100& 0.9948&0.0013&0.6822&0.1890 \\
         Seg. size 1000&0.9812&0.0010&0.8682&0.2928\\
         Seg. size 10000&0.8791&0.0068&0.9303&0.0675\\
         \midrule
         \multicolumn{5}{c}{\textbf{Max events test}} \\
         \midrule
         Seg. size 100&0.9923& 0.0980&0.8291&0.0929\\
         Seg. size 1000&0.9769&0.0821&0.9043&0.2425\\
         Seg. size 10000&0.8577&0.1518&0.9386&0.3258\\
         \midrule
         \multicolumn{5}{c}{\textbf{Number of provisioner organizations test}} \\
         \midrule
         Seg. size 100&0.9884&0.3184&0.8577&0.5103\\
         Seg. size 1000&0.9799&0.5174&0.7902&0.5211\\
         Seg. size 10000&0.9521&0.6102&0.6977&0.6101\\
         \bottomrule
    \end{tabular}
    }
  } 


==> content/tables/eventLogs.tex <==
%    \begin{minipage}[t]{1\linewidth}
    %\subfloat{% Subtable 1
       \resizebox{\textwidth}{!}{%
            \begin{tabular}{l l S[table-format = 2.0] S[table-format = 4.0] S[table-format = 3.0] S[table-format = 1.0] S[table-format = 2.0] l} \toprule
 %           	                &   &  & &  \multicolumn{3}{c}{\textbf{Trace length}} &                        \\ \cmidrule{5-7}
            	\textbf{Name}               & \textbf{Type} & \textbf{Activities} & \textbf{Cases} & \textrm{\textbf{Max} events} & \textrm{\textbf{Min} events} & \textrm{\textbf{Avg}.\ events} & \textbf{Organization $\mapsto$ Activities}                        \\ \midrule
            	Motivating scenario  & Synthetic     & 19                  & 1000           &18 &9 &14 & ${\Org}^P \mapsto 3$, ${\Org}^C \mapsto 5$, ${\Org}^H \mapsto 14$ \\
            	Sepsis~\citep{seps}                       & Real          & 16                & 1050          & 185 & 3 & 15  & ${\Org}^1 \mapsto 1$, ${\Org}^2 \mapsto 1$, ${\Org}^3 \mapsto 14$ \\                                                                 
            	BPIC2013~\citep{bpic2013}                   & Real          & 7                  & 1487           &123 &1 &9 & ${\Org}^1 \mapsto 6$, ${\Org}^2 \mapsto 7$, ${\Org}^3 \mapsto 6$  \\ \bottomrule& & 
            \end{tabular}
        }% resizebox
    %}% subfloat
%    \end{minipage}%

==> template/Makefile <==
# LATEX: pdflatex | xelatex | lualatex
LATEX = lualatex
LATEX_FLAGS = -shell-escape
BIBTEX = bibtex

FILES = $(patsubst %.tex, %.pdf, $(wildcard *.tex))

all: $(FILES)


%.pdf: %.tex
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	-$(BIBTEX) `basename $< .tex`
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	$(LATEX) $(LATEX_FLAGS) $<
	qpdf --linearize --newline-before-endstream $@ /tmp/$@
	mv /tmp/$@ $@

clean:
	-rm -f *.{log,toc,tac,aux,dvi,ps,bbl,blg,tmp,nav,out,snm,vrb,rel,cut,abs,xmpi,xmpdata,*~}
	-rm -rf out _minted* auto
	for i in $(ALLSUBDIRS); do \
	    (cd $$i; make clean) || exit 1; \
	done
	-rm $(FILES)

cleanall: clean
	-rm -rf out auto
